A Scalable Heuristic for Viral Marketing Under the Tipping Model

In a "tipping" model, each node in a social network, representing an individual, adopts a property or behavior if a certain number of his incoming neighbors currently exhibit the same. In viral marketing, a key problem is to select an initial "seed" set from the network such that the entire network adopts any behavior given to the seed. Here we introduce a method for quickly finding seed sets that scales to very large networks. Our approach finds a set of nodes that guarantees spreading to the entire network under the tipping model. After experimentally evaluating 31 real-world networks, we found that our approach often finds seed sets that are several orders of magnitude smaller than the population size and outperform nodal centrality measures in most cases. In addition, our approach scales well - on a Friendster social network consisting of 5.6 million nodes and 28 million edges we found a seed set in under 3.6 hours. Our experiments also indicate that our algorithm provides small seed sets even if high-degree nodes are removed. Lastly, we find that highly clustered local neighborhoods, together with dense network-wide community structures, suppress a trend's ability to spread under the tipping model.

==> alg.tex <==
\section{Algorithms}
\label{alg-sec}

In this section, we introduce an integer program that solved the MIN-SEED problem exactly and our new decomposition-based heuristic.

\subsection{Exact Approach}

Below we present SEED-IP, an integer program that if solved exactly, guarantees an exact solution to MIN-SEED (see Proposition~\ref{ip-corr}).  Though, in general, solving an integer program is also NP-hard, suggesting that an exact solution will likely take exponential time, good approximation techniques such as branch-and-bound exist and mature tools such as QSopt and CPLEX can readily take and approximate solutions to integer programs.

\begin{definition}[SEED-IP]
\begin{eqnarray}
\label{objFcn}& \min \sum_i x_{i,1},\,\,\,\,\,\,\,\,\,\,	 \mathit{w.r.t.}\\
\label{varConst}\forall i,t \in \{1,\ldots, n\}, & x_{i,t} \in \{0, 1\}  \\
\label{endConst}\forall i, & x_{i,n} = 1 \\
\label{actConst}\forall i, \forall t >0,&\,\,\,\,\,\,\,\,\,\, x_{i,t} \leq x_{i,t-1}+ \frac{1}{d^{in}_i \theta(v_i)}\sum_{v_j \in \eta^{in}_i}x_{j,t-1}
\end{eqnarray}
\end{definition}

\begin{proposition}
\label{ip-corr}
If $V'$ is a solution to MIN-SEED, then setting $\forall v_i \in V', x_{i,1}=1$ and $\forall v_i \notin V', x_{i,1}=0$ is a solution to SEED-IP.\\
If the vector $[x_{i,t}]$ is a solution to SEED-IP, then $\{ v_i | x_{i,1}=1\}$ is a solution to MIN-SEED.
\end{proposition}
\begin{proof}
\noindent Claim 1: If $V'$ is a solution to MIN-SEED, then setting $\forall v_i \in V', x_{i,1}=1$ and $\forall v_i \notin V', x_{i,1}=0$ is a solution to SEED-IP.\\
Let $[x_{i,t}]$ be a vector for SEED-IP created as per claim 1.  Suppose, by way of contradiction (BWOC), there exists vector $[x'_{i,t}]$ s.t. $\sum_i x'_{i,1} < \sum_i x_{i,1}$.  However, consider the set of nodes $V'' = \{ v_i | x'_{i,1}=1\}$.  By Constraint~\ref{actConst} of SEED-IP, we know that, for $t >1$, that if $x'_{i,t} = 1$, we have $v_i \in A^t_\theta(V'')$.  Hence, by Constaint~\ref{endConst} $V''$ is a solution to MIN-SEED.  This means that $|V''| < |V'|$ as $\sum_i x'_{i,1} < \sum_i x_{i,1}$, which is a contradiction.\\
\noindent Claim 2: If the vector $[x_{i,t}]$ is a solution to SEED-IP, then $\{ v_i | x_{i,1}=1\}$ is a solution to MIN-SEED.\\
Suppose, BWOC, there exists set $V''$ that is a solution to MIN-SEED s.t. $|V''| < |\{ v_i | x_{i,1}=1\}|$.  Consider the vector $[x'_{i,t}]$ where $\forall i,$ $x'_{i,0}=1$ iff $v_i \in V''$.  By Constraint~\ref{actConst} of SEED-IP, we know that, for $t >1$, that if $v_i \in A^t_\theta(V'')$, we have $x'_{i,t} = 1$.  Hence, as $A^t_\theta(V'') = V$, know that $[x'_{i,t}]$  satisfies Constraint~\ref{endConst}.  Hence, as $|V''| < |\{ v_i | x_{i,1}=1\}|$, we know $\sum_i x'_{i,1} < \sum_i x_{i,1}$, which is a contradiction.\\
\noindent Proof of theorem: Follows directly form claims 1-2.
\end{proof}

However, despite the availability of approximate solvers, SEED-IP requires a quadratic number of variables and constraints (Proposition~\ref{numConst}), which likely will prevent this approach from scaling to very large datasets.  As a result, in the next section we introduce our heuristic approach.

\begin{proposition}
\label{numConst}
SEED-IP requires $n^2$ variables and $2n^2$ constraints.
\end{proposition}


\subsection{Heuristic}

To deal with the intractability of the MIN-SEED problem, we design an algorithm that finds a non-trivial subset of nodes that causes the entire graph to  activate, but we do not guarantee that the resulting set will be of minimal size.  The algorithm is based on the idea of shell decomposition often cited in physics literature~\cite{Seidman83,ShaiCarmi07032007,InfluentialSpreaders_2010,baxter11} but modified to ensure that the resulting set will lead to all nodes being activated.  The algorithm, \textsf{TIP\_DECOMP} is presented in this section.

\algsetup{indent=1em}
	\begin{algorithm}[h!]
		\caption{ \textsf{TIP\_DECOMP}}
		\begin{algorithmic}[1]


		\REQUIRE Threshold function, $ \theta $ and directed social network $G=(V,E)$
		\ENSURE $ V' $
		\medskip

		\STATE{ For each vertex $ v_i $, compute $ k_i $}.
		\STATE{ For each vertex $ v_i,\ dist_i = d_i^{in} - k_i $}.
		\STATE{ FLAG = TRUE}.
		\WHILE{ FLAG }
			\STATE {Let $ v_i $ be the element of $ v $ where $ dist_i $ is minimal}.
			\IF { $ dist_i = \infty $}
				\STATE{ FLAG = FALSE}.
			\ELSE
				\STATE{ Remove $ v_i $ from $G$ and for each $ v_j $ in $ \eta_i^{out} $, if $dist_j > 0$, set
				$  dist_j = dist_j-1 $.  Otherwise set $dist_j = \infty $}.
			\ENDIF
		\ENDWHILE
		\RETURN{ All nodes left in $ G $}.
	\end{algorithmic}
\end{algorithm}


Intuitively, the algorithm proceeds as follows (Figure 1).  Given network $G=(V,E)$ where each node $v_i$ has threshold $k_i = \lceil \theta (v_i) \cdot d^{in}_i \rceil$, at each iteration, pick the node for which $d^{in}_i - k_i$ is the least but positive (or $0$) and remove it.  Once there are no nodes for which $d^{in}_i - k_i$ is positive (or $0$), the algorithm outputs the remaining nodes in the network.  

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/fig1}
    \end{center}
\caption{Example of our algorithm for a simple network depicted in box \textbf{A}.  We use a threshold value set to $50\%$ of the node degree.  Next to each node label (lower-case letter) is the value for $d^{in}_i - k_i$ (where $k_i = \lceil \frac{d^{in}_i}{2} \rceil$).  In the first four iterations, nodes e, f, h, and i are removed resulting in the network in box \textbf{B}.  This is followed by the removal of node j resulting in the network in box \textbf{C}.  In the next two iterations, nodes a and b are removed (boxes \textbf{D}-\textbf{E} respectively).  Finally, node c is removed (box \textbf{F}).  The nodes of the final network, consisting of d and g, have negetive values for $d_i-\theta_i$ and become the output of the algorithm.}
    %\label{main-fig}
\end{figure}


Now, we prove that the resulting set of nodes is guaranteed to cause all nodes in the graph to activate under the tipping model.  This proof follows from the fact that any node removed is activated by the remaining nodes in the network.  

\begin{theorem}
If all nodes in $ V'\ \subseteq\ V $ returned by \textsf{TIP\_DECOMP} are initially active, then every node in $ V $ will eventually be activated, too. 
\end{theorem}

\begin{proof}
Let $ w $ be the total number of nodes removed by \textsf{TIP\_DECOMP}, where $ v_1 $ is the last node removed and $ v_w $ is the first node removed.  We prove the theorem by induction on $ w $ as follows.  We use $P(w)$ to denote the inductive hypothesis which states that all nodes from $ v_1 $ to $ v_w $ are active. In the base case, $P(1)$ trivially holds as we are guaranteed that from set $V'$ there are at least $k_1$ edges to $v_1$ (or it would not be removed).  For the inductive step, assuming $P(w)$ is true, when $ v_{w+1} $ was removed from the graph $ dist_{w+1} \geq 0 $ which means that $ d_{w+1}^{in} \geq k_{w+1} $.  All nodes in $\eta^{in}_{w+1}$ at the time when $ v_{w+1} $ was removed are now active, so $ v_{w+1} $ will now be activated - which completes the proof.
\end{proof}

We also note that by using the appropriate data structure (we used a binomial heap in our implementation), for a network of $n$ nodes and $m$ edges, this algorithm can run in time $O(m \log n)$.

\begin{proposition}
\label{tcomp}
The complexity of \textsf{TIP\_DECOMP} is $ O(m \cdot log(n)) $.
\end{proposition}
\begin{proof}
If we use a binomial heap as described in \cite{cormen}, we can create a heap where we store each node and assign it a key value of $dist_i$ for each node $v_i$.  The creation of a heap takes constant time and inserting the $n$ vertices will take $O(n log(n))$ time.  We can also maintain a list data structure as well.  In the course of the while loop, all nodes will either be removed (as per the algorithm), decreased in key-value no more than $d^{in}_i$ or increased to infinity (which we can implement as being removed and added to the list).  Hence, the number of decrease key or removal operations is bounded by $n+\sum_i d^{in}_i$.  As $\sum_i d^{in}_i = m$ (where $m$ is the number of edges).  As $ O(m \cdot log(n)) $, the statement follows.
\end{proof}

==> concl.tex <==
\section{Conclusion}

As recent empirical work on tipping indicates that it can occur in real social networks,\cite{centola10,zhang11} our results are encouraging for viral marketers.  Even if we assume relatively large threshold values, small initial seed sizes can often be found using our fast algorithm - even for large datasets.  For example, with the FourSquare online social network, under majority threshold ($50\%$ of incoming neighbors previously adopted), a viral marketeer could expect a $297$-fold return on investment.  As results of this type seem to hold for many online social networks, our algorithm seems to hold promise for those wishing to ``go viral.''


==> exp2.tex <==
\section{Results}
\label{res-sec}
In this section we describe the results of our experimental evaluation.  We describe the datasets we used for the experiments in Section~\ref{ds-sec}.  We evaluate the run-time of \textsf{TIP\_DECOMP} in Section~\ref{rt-sec}.  In Section~\ref{ss-sec}, we evaluate the size of the seed-set returned by the algorithm and we compare this to the seed size returned by known centrality measures in Section~\ref{cent-sec}.  We then study how the removal of high-degree nodes and community structure affect the results of the algorithm in Sections~\ref{robust-sec} and \ref{comm-sec} respectively.

The algorithm \textsf{TIP\_DECOMP} was written using Python 2.6.6 in 200 lines of code that leveraged the NetworkX library available from http://networkx.lanl.gov/.  The code used a binomial heap library written by Bj\"orn B. Brandenburg available from http://www.cs.unc.edu/$\sim$bbb/.  The experiments were run on a computer equipped with an Intel X5677 Xeon Processor operating at 3.46 GHz with a 12 MB Cache running Red Hat Enterprise Linux version 6.1 and equipped with 70 GB of physical memory.  All statistics presented in this section were calculated using R 2.13.1.


\subsection{Datasets}
\label{ds-sec}

In total, we examined $31$ networks: nine academic collaboration networks, three e-mail networks, and $19$ networks extracted from social-media sites.  The sites included included general-purpose social-media (similar to Facebook or MySpace) as well as special-purpose sites (i.e. focused on sharing of blogs, photos, or video).

All datasets used in this paper were obtained from one of four sources: the ASU Social Computing Data Repository,~\cite{Zafarani+Liu:2009} the Stanford Network Analysis Project,~\cite{snap} the University of Michigan,~\cite{umich} and Universitat Rovira i Virgili.\cite{uvi}  All networks considered were symmetric -- i.e. if a directed edge from vertex $v$ to $v'$ exists, there is also an edge from vertex $v'$ to $v$.  Tables~\ref{fig3} (A-C) show some of the pertinent qualities of these networks.  The networks are categorized by the results for the MIN-SEED experiments (explained later in this section).  In what follows, we provide their real-world context.

\subsubsection{Category A}
\begin{itemize}
\item{\textbf{BlogCatalog} is a social blog directory that allows users to share blogs with friends.~\cite{Zafarani+Liu:2009}  The first two samples of this site, BlogCatalog1 and 2, were taken in Jul. 2009 and June 2010 respectively.  The third sample, BlogCatalog3 was uploaded to ASU's Social Computing Data Repository in Aug. 2010.}
\item{\textbf{Buzznet} is a social media network designed for sharing photographs, journals, and videos.~\cite{Zafarani+Liu:2009}  It was extracted in Nov. 2010.}
\item{\textbf{Douban } is a Chinese social medial website designed to provide user reviews and recommendations.~\cite{Zafarani+Liu:2009}  It was extracted in Dec. 2010.}
\item{\textbf{Flickr} is a social media website that allows users to share photographs.~\cite{Zafarani+Liu:2009}  It was uploaded to ASU's Social Computing Data Repository in Aug. 2010.}
\item{\textbf{Flixster} is a social media website that allows users to share reviews and other information about cinema.~\cite{Zafarani+Liu:2009}  It was extracted in Dec. 2010.}
\item{\textbf{FourSquare} is a location-based social media site.~\cite{Zafarani+Liu:2009}  It was extracted in Dec. 2010.}
\item{\textbf{Frienster} is a general-purpose social-networking site.~\cite{Zafarani+Liu:2009} It was extracted in Nov. 2010.}
\item{\textbf{Last.Fm} is a music-centered social media site.~\cite{Zafarani+Liu:2009} It was extracted in Dec. 2010.}
\item{\textbf{LiveJournal} is a site designed to allow users to share their blogs.~\cite{Zafarani+Liu:2009}  It was extracted in Jul. 2010.}
\item{\textbf{Livemocha} is touted as the ``world's largest language community.''~\cite{Zafarani+Liu:2009}  It was extracted in Dec. 2010.}
\item{\textbf{WikiTalk} is a network of individuals who set and received messages while editing WikiPedia pages.~\cite{snap}  It was extracted in Jan. 2008.}
\end{itemize}

\subsubsection{Category B}
\begin{itemize}
\item{\textbf{Delicious} is a social bookmarking site, designed to allow users to share web bookmarks with their friends.~\cite{Zafarani+Liu:2009} It was extracted in Dec. 2010.}
\item{\textbf{Digg} is a social news website that allows users to share stories with friends.~\cite{Zafarani+Liu:2009}  It was extracted in Dec. 2010.}
\item{\textbf{EU E-Mail} is an e-mail network extracted from a large European Union research institution.~\cite{snap}  It is based on e-mail traffic from Oct. 2003 to May 2005.}
\item{\textbf{Hyves} is a popular general-purpose Dutch social networking site.~\cite{Zafarani+Liu:2009}  It was extracted in Dec. 2010.}
\item{\textbf{Yelp} is a social networking site that allows users to share product reviews.~\cite{Zafarani+Liu:2009}  It was extracted in Nov. 2010.}
\end{itemize}

\subsubsection{Category C}
\begin{itemize}
\item{\textbf{CA-AstroPh} is a an academic collaboration network for Astro Physics from Jan. 1993 - Apr. 2003.~\cite{snap}}
\item{\textbf{CA-CondMat} is an academic collaboration network for Condense Matter Physics.  Samples from 1999 (CondMat99), 2003 (CondMat03), and 2005 (CondMat05) were obtained from the University of Michigan.~\cite{umich}  A second sample from 2003 (CondMat03a) was obtained from Stanford University.~\cite{snap}}
\item{\textbf{CA-GrQc} is a an academic collaboration network for General Relativity and Quantum Cosmology from Jan. 1993 - Apr. 2003.~\cite{snap}}
\item{\textbf{CA-HepPh} is a an academic collaboration network for High Energy Physics - Phenomenology from Jan. 1993 - Apr. 2003.~\cite{snap}}
\item{\textbf{CA-HepTh} is a an academic collaboration network for High Energy Physics - Theory from Jan. 1993 - Apr. 2003.~\cite{snap}}
\item{\textbf{CA-NetSci} is a an academic collaboration network for Network Science from May 2006.}
\item{\textbf{Enron E-Mail} is an e-mail network from the Enron corporation made public by the Federal Energy Regulatory Commission during its investigation.~\cite{snap}}
\item{\textbf{URV E-Mail} is an e-mail network based on communications of members of the University Rovira i Virgili (Tarragona).~\cite{uvi}  It was extracted in 2003.}
\item{\textbf{YouTube} is a video-sharing website that allows users to establish friendship links.~\cite{Zafarani+Liu:2009}  The first sample (YouTube1) was extracted in Dec. 2008.  The second sample (YouTube2) was uploaded to ASU's Social Computing Data Repository in Aug. 2010.}
\end{itemize}

\begin{table}[ht]
     \begin{center}
        \includegraphics[width=.8\linewidth]{ieee-tables}
    \end{center}
    \caption{Information on the networks in Categories A, B, and C.}
    \label{fig3}
\end{table}


\begin{table}[ht]
     \begin{center}
        \includegraphics[width=.8\linewidth]{figures/dirInfoTable}
    \end{center}
    \caption{TOADD, TEXT, REF TO FIG ALSO}
    \label{dirInfo}
\end{table}



\subsubsection{Runtime}
\label{rt-sec}
First, we examined the runtime of the algorithm (see Figures~\ref{figRt} and Table~\ref{firRtTable).  Our experiments aligned well with our time complexity result (Proposition~\ref{tcomp}).  For example, a network extracted from the Dutch social-media site Hyves consisting of $1.4$ million nodes and $5.5$ million directed edges was processed by our algorithm in at most $12.2$ minutes.  The often-cited LiveJournal dataset consisting of $2.2$ million nodes and $25.6$ million directed edges was processed in no more than $66$ minutes - a short time to approximate an NP-hard combinatorial problem on a large-sized input.

\begin{figure}[htbb]
    \begin{center}
        \includegraphics[width=.89\linewidth]{runtimeGph}
    \end{center}
    \caption{$m \ln n$ vs. runtime in seconds (log scale, $m$ is number of edges, $n$ is number of nodes).  The relationship is linear with $R^2=0.9015$, $p=2.2 \cdot 10^{-16}$.}
    \label{figRt}
\end{figure}

\begin{table}[ht]
     \begin{center}
        \includegraphics[width=.8\linewidth{figures/runtimeTable}
    \end{center}
    \caption{TOADD, TEXT, REF TO FIG ALSO}
    \label{figRtTable}
\end{table}


\subsubsection{Seed Size}
\label{ss-sec}
For each network, we performed $10$ ``integer'' trials.  In these trials, we set $\theta(v_i)=\min(d^{in}_i,k)$ where $k$ was kept constant among all vertices for each trial and set at an integer in the interval $[1,10]$.  We evaluated the ability of a network to promote spreading under the tipping model based on the size of the set of nodes returned by our algorithm (as a percentage of total nodes).  For purposes of discussion, we have grouped our networks into three categories based on results (Figure~\ref{figFirst} and Table~\ref{figX}).  In general, online social networks had the smallest seed sets - $13$ networks of this type had an average seed set size less than $2\%$ of the population (these networks were all in Category A).  We also noticed, that for most networks, there was a linear realtion between threshold value and seed size.

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/fig2}
    \end{center}
       \caption{Threshold value (assigned as an integer in the interval $[1,10]$) vs. size of initial seed set as returned by our algorithm in our three identified categories of networks (categories A-C are depicted in panels A-C respectively).  Average seed sizes were under $2\%$ for Categorty A, $2-10\%$ for Category B and over $10\%$ for Category C.  The relationship, in general, was linear for categories A and B and lograthimic for C.  CA-NetSci had the largest Louvain Modularity and clustering coefficient of all the networks.  This likely explains why that particular network seems to inhibit spreading.}
    \label{figFirst}
\end{figure}

Category A can be thought of as social networks highly susceptible to influence - as a very small fraction of initially activated individuals can lead to activation of the entire population.  All were extracted from social media websites.  For some of the lower threshold levels, the size of the set of seed nodes was particularly small.  For a threshold of three, $11$ of the Category A networks produced seeds smaller than $0.5\%$ of the total populationa.  For a threshold of four, nine networks met this criteria.

Networks in Category B are susceptible to influence with a relatively small set of initial nodes - but not to the extent of those in Category A.  They had an average initial seed size greater than $2\%$ but less than $10\%$. Members in this group included two general purpose social media networks, two specialty social media networks, and an e-mail network.

Category C consisted of networks that seemed to hamper diffusion in the tipping model, having an average initial seed size greater than $10\%$.  This category included all of the academic collaboration networks, two of the email networks, and two networks derived from friendship links on YouTube.

We also studied the effects on spreading when the threshold values were assigned as a specific fraction of each node's in-degree~\cite{jy05,wattsDodds07}, which results in heterogeneous $\theta_i$'s across the network.  We performed $12$ trials for each network.  Thresholds for each trial were based on the product of in-degree and a fraction in the interval $[0.05,0.60]$ (multiples of $0.05$).  The results (Figure~\ref{figFrac} and Table~\ref{figX}) were analogous to our integer tests.  We also compared the averages over these trials with $M$ and $C$ and obtained similar results as with the other trials (Figure~\ref{main-fig} B).

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/fig4}
    \end{center}
   \caption{Threshold value (assigned as a fraction of node in-degree as a multiple of $0.05$ in the interval $[0.05,0.60]$) vs. size of initial seed set as returned by our algorithm in our three identified categories of networks (categories A-C are depicted in panels A-C respectively, categories are the same as in Figure 1). Average seed sizes were under $5\%$ for Categorty A, $1-7\%$ for Category B and over $3\%$ for Category C.  In general, the relationship between threshold and initial seed size for networks in all categories was exponential.}
    \label{figFrac}
\end{figure}

\subsection{Tests on Non-Symmetric Networks}

NEED TO ADD TEXT \ref{figNonSym}

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/dirTest}
    \end{center}
   \caption{TOADD}
    \label{figNonSym}
\end{figure}



\subsection{Comparison with Centrality Measures}
\label{cent-sec}

We compared our results with three popular centrality measures: degree, betweenness, and closeness.  Here, we define degree centrality is simply the number of outgoing adjacent nodes.~\footnote{Note that as our examined networks were symmetric, our empirical results hold for the number of incoming adjacent edges as well as the total number of adjacent edges.}  The intuition behind high betweenness centrality nodes is that they function as ``bottlenecks'' as many paths in the network pass through them.  Hence, betweenness is a medial centrality measure.  Let $\sigma_{st}$ be the number of shortest paths between nodes $s$ and $t$ and $\sigma_{st}(v)$ be the number of shortest paths between $s$ and $t$ containing node $v$.  In \cite{freeman77}, betweenness centrality for node $v$ is defined as $\sum_{s\neq v \neq t}\frac{\sigma_{st}(v)}{\sigma_{st}}$.  In most implementations, including the ones used in this paper, the algorithm of \cite{brandes01} is used to calculate betweenness centrality.  Another common measure from the literature that we examined is closeness ~\cite{freeman79cent}.  Given node $i$, its closeness $C_c(i)$ is the inverse of the average shortest path length from node $i$ to all other nodes in the graph. Intuitively, closeness measures how ``close'' it is to all other nodes in a network.  Formally, if we define the shortest path between nodes $i$ to $j$ as function $d_G(i,j)$, we can express the average path length from $i$ to all other nodes as 
\begin{equation}
L_i = \frac{\sum_{j\in V\setminus i} d_G(i,j)}{|V|-1}.
\end{equation}
Hence, the closeness of a node can be formally written as 
\begin{equation}
C_c  (i) = \frac{1}{L_i} = \frac{|V|-1}{\sum_{j\in V\setminus i} d_G(i,j)}.
\end{equation}
A more complete discussion of centrality measures can be found in \cite{wasserman1994social}.

We evaluated the performance of centrality measures in finding a seed set by iteratively selecting the most central nodes with respect to a given measure until the $\Gamma_\theta$ of that set returns the set of all nodes.  Due to the computational overhead of calculating these centrality measures and the repeated re-evaluation of $\Gamma_\theta$, we limited this comparison to only \textbf{BlogCatalog3}, \textbf{CA-HepTh}, \textbf{CA-NetSci}, \textbf{URV E-Mail}, and \textbf{Douban} (degree and closeness only).  As with the experiments in the previous section, we studied threshold settings based on an integer in the interval $[1,10]$ (see Figure~\ref{centInt}) and as a fraction of incoming neighbors in the interval $[0.05,0.60]$ (multiples of $0.05$, see Figure~\ref{centFrac}).  In general, selecting highly-central nodes is an inefficient method for finding small seed sets.

In all but the lowest threshold settings, the use of centrality measures for the integer-threshold trials proved to significantly underperformed when the method presented in this paper - often returning seed-sets several orders of magnitude larger and in many cases including the majority of nodes in the network.

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/intCent}
    \end{center}
   \caption{The use of degree, betweenness and closeness to find seed-sets on select networks when the threshold is set to an integer in the interval $[1,10]$.  For these trials, centrality measure returned significantly larger (several orders of magnitude) larger seed sets than our approach.}
    \label{centInt}
\end{figure}

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/specInt}
    \end{center}
   \caption{TOADD AND TEXT DESC AND TEXT FIG REF}
    \label{specInt}
\end{figure}



Our tests using fractional-based thresholds tell a slightly different story.  While our method still significantly outperformed the centrality measures on the collaboration networks, this was not always the case with the other networks.  Specifically, the online social network \textbf{BlogCatalog3} and e-mail network \textbf{URV E-Mail}, outperformed our method for many fraction-based threshold settings.  However, we note that for \textbf{URV E-Mail} the centrality measures provide a seed set more than double in size than that returned by \textsf{TIP\_DECOMP}.  Additionally, though centrality measures outperformed \textsf{TIP\_DECOMP} for \textbf{BlogCatalog3}, this does not appear to hold for all social networks as the seed sets returned using centrality measures for the \textsf{Douban} approaches at least an order of magnitude increase over our method for nearly every fractional threshold setting for all centrality measures.  Hence, we conclude that for fraction-based thresholds, using centrality measures to find seed sets provides inconsistent results, and when it fails, it tends to provide a large portion of the network.  A possibility for a practical algorithm that could combine both methods would be to first run \textsf{TIP\_DECOMP}, returning some set $V'$.  Then, create set $V''$ by selecting the most central nodes until either $|V'| = |V''|$ or $\Gamma_\theta(V'')=V$ (whichever ensures the lower cardinality for $V''$.  If $|V'| = |V''|$, return $V'$, otherwise return $V''$.  For such an approach, we would likely recommend using degree centrality due to its ease of computation and performance in our experiments.  However, we note that highly-central nodes often may not be realistic targets for a viral-marketing campaign.  For instance, it may be cost-prohibitive to create a seed set consisting of major celebrities in order to spread the use of a product.  As such is a practical concern, we look at the performance of \textsf{TIP\_DECOMP} when high-degree nodes are removed in the next section.

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/fracCent}
    \end{center}
   \caption{The use of degree, betweenness and closeness to find seed-sets on select networks when the threshold is set to an fraction in the interval $[0.05,0.60]$ (multiples of $0.05$).}
    \label{centFrac}
\end{figure}

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/specPerc}
    \end{center}
   \caption{TOADD AND TEXT DESC AND TEXT FIG REF}
    \label{specFrac}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Effect on the Speed of the Diffusion Process}

TO ADD TEXT

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/durationTest}
    \end{center}
   \caption{TOADD AND TEXT DESC AND TEXT FIG REF}
    \label{durTest}
\end{figure}

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/greatestSingleIncr}
    \end{center}
   \caption{TOADD AND TEXT DESC AND TEXT FIG REF}
    \label{grtSingIncr}
\end{figure}


\subsection{Effect of Removing High-Degree Nodes}
\label{robust-sec}

In the last section we noted that high-degree nodes may not always be targetable in a viral marketing campaign (i.e. it may be cost prohibitive to include them in a seed set).  In this section, we explore the affect of removing high-degree nodes on the size of the seed-set returned by \textsf{TIP\_DECOMP}.  In these trials, we studied all $31$ networks and looked at two specific threshold settings: an integer threshold of $2$ (Figure~\ref{twoRemTest}) and a fractional threshold of $0.5$ (Figure~\ref{fifRemTest}).  We then studied the effect of removing up to $50\%$ of the nodes in order from greatest to least degree.

With an integer threshold of $2$, networks in category A still retained a seed-size (as returned by \textsf{TIP\_DECOMP}) two orders of magnitude smaller than the population size up to the removal of $10\%$ of the top degree nodes, and for many networks this was maintained to $50\%$.  Networks in category B retained seed sets an order of magnitude smaller than the population for up to $50\%$ of the nodes removed.  For most networks in category C, the seed size remained about a quarter of the population size up to $15\%$ of the top degree nodes being removed.

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/twoRem}
    \end{center}
   \caption{Size of the seed set returned by \textsf{TIP\_DECOMP} (as a fraction of the popualtion) as a function of the percent of the highest degree nodes removed from the network with an integer theshold of $2$ for networks in categories A-C.}
    \label{twoRemTest}
\end{figure}

With a fractional threshold of $0.5$, we noted that many networks in category A actually had larger seed sets (as returned by \textsf{TIP\_DECOMP}) when more high degree nodes are removed.  Further, networks in categories A-B retained seed sets of at least an order of magnitude smaller than the population in these tests while most networks in category C retained sizes of about a quarter of the population.

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/fifRem}
    \end{center}
   \caption{Size of the seed set returned by \textsf{TIP\_DECOMP} (as a fraction of the popualtion) as a function of the percent of the highest degree nodes removed from the network with an fractional theshold of $0.5$ for networks in categories A-C.}
    \label{fifRemTest}
\end{figure}


\subsubsection{Seed Size as a Function of Community Structure}
\label{comm-sec}

In this section, we view the results of our heuristic algorithm as a measurement of how well a given network promotes spreading.  Here, we use this measurement to gain insight into which structural aspects make a  network more likely to be ``tipped.''  We compared our results with two network-wide measures characterizing community structure.  First, clustering coefficient ($C$) is defined for a node as the fraction of neighbor pairs that share an edge - making a triangle.  For the undirected case, we define this concept formally below.

\begin{definition}[Clustering Coefficient]
Let $ r $ be the number of edges between nodes with which $ v_i $ has an edge and $d_i$ be the degree of $v_i$.  The \textbf{clustering coefficient}, $ C_i = \dfrac {2r}  {d_i(d_i - 1)} $.
\end{definition}

Intuitively, a node with high $C_i$ tends to have more pairs of friends that are also mutual friends.  We use the average clustering coefficient as a network-wide measure of this local property.

Second, we consider modularity ($M$) defined by Newman and Girvan.~\cite{newman04}.  For a partition of a network, $M$ is a real number in $[-1,1]$ that measures the density of edges within partitions compared to the density of edges between partitions.  We present a formal definition for an undirected network below.

\begin{definition}[Modularity~\cite{newman04}]
\textbf{Modularity}, $ M = \dfrac 1 {2m} \sum_{i,j \in V} [1 - \dfrac {d_i d_j} {2m}] \delta (c_i, c_j) $, where $m$ is the number of undirected edges, $d_i$ is node degree, $ c_i $ is the community to which $ v_i $ belongs and $ \delta (x, y) = 1 $ if $ x = y $ and $ 0 $ otherwise.
\end{definition}

The modularity of an optimal network partition can be used to measure the quality of its community structure.  Though modularity-maximization is NP-hard, the approximation algorithm of Blondel et al.~\cite{blondel08} (a.k.a. the ``Louvain algorithm'') has been shown to produce near-optimal partitions.\footnote{Louvain modularity was computed using the implementation available from CRANS at  http://perso.crans.org/aynaud/communities/.}  We call the modularity associated with this algorithm the ``Louvain modularity.''  Unlike the $C$, which describes local properties, $M$ is descriptive of the community level.  For the $31$ networks we considered, $M$ and $C$  appear uncorrelated ($R^2 = 0.0538$, $p=0.2092$).

We plotted the initial seed set size ($S$) (from our algorithm - averaged over the $10$ threshold settings) as a function of $M$ and $C$ (Figure~\ref{main-fig}a) and uncovered a correlation (planar fit, $R^2=0.8666$, $p=5.666 \cdot 10^{-13}$, see Figure~\ref{main-fig} A).  The majority of networks in Category C (less susceptible to spreading) were characterized by relatively large $M$ and $C$ (Category C includes the top nine networks w.r.t. $C$ and top five w.r.t. $M$).  Hence, networks with dense, segregated, and close-knit communities (large $M$ and $C$) suppress spreading.  Likewise, those with low $M$ and $C$ tended to promote spreading.  Also, we note that there were networks that promoted spreading with dense and segregated communities, yet were less clustered (i.e. Category A networks Friendster and LiveJournal both have $M\geq 0.65$ and $C \leq 0.13$).  Further, some networks with a moderately large clustering coefficient were also in Category A (two networks extracted from BlogCatalog had $C\geq 0.46$) but had a relatively less dense community structure (for those two networks $M \leq 0.33$).

\begin{figure}
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/fig3}
    \end{center}
    \caption{\textbf{(A)} Louvain modularity ($M$) and average clustering coefficient ($C$) vs. the average seed size ($S$).  The planar fit depicted is $S=43.374 \cdot M +  33.794 \cdot C - 24.940$ with $R^2=0.8666$, $p=5.666 \cdot 10^{-13}$.  \textbf{(B)} Same plot at (A) except the averages are over the 12 percentage-based threshold values.  The planar fit depicted is $S=18.105 \cdot M + 17.257 \cdot C - 10.388$ with $R^2=0.816$, $p=5.117 \cdot 10^{-11}$.}
    \label{main-fig}
\end{figure}


\begin{table}[ht]
     \begin{center}
        \includegraphics[width=.8\linewidth]{ieee-tables-2}
    \end{center}
    \caption{Regression analysis and network-wide measures for the networks in Categories A, B, and C.}
    \label{figX}
\end{table}

\begin{table}[ht]
     \begin{center}
        \includegraphics[width=.8\linewidth]{figures/dirResTable}
    \end{center}
      \caption{TOADD AND TEXT DESC AND TEXT FIG REF}
    \label{dirResTable}
\end{table}


==> rw.tex <==
\section{Related Work}
\label{rw-sec}
Tipping models first became popular by the works of \cite{Gran78} and \cite{Schelling78} where it was presented primarily in a social context.  Since then, several variants have been introduced in the literature including the non-deterministic version of \cite{kleinberg} (described later in this section) and a generalized version of \cite{jy05}.  In this paper we focused on the deterministic version.  In \cite{wattsDodds07}, the authors look at deterministic tipping where each node is activated upon a percentage of neighbors being activated.  Dryer and Roberts \cite{Dreyer09} introduce the MIN-SEED problem, study its complexity, and describe several of its properties w.r.t. certain special cases of graphs/networks.  The hardness of approximation for this problem is described in \cite{chen09siam}.  The work of \cite{benzwi09} presents an algorithm for target-set selection whose complexity is determined by the tree-width of the graph - though it provides no experiments or evidence that the algorithm can scale for large datasets.  The recent work of \cite{reichman12} proves a non-trivial upper bound on the smallest seed set.

Our algorithm is based on the idea of shell-decomposition that currently is prevalent in physics literature.  In this process, which was introduced in \cite{Seidman83}, vertices (and their adjacent edges) are iteratively pruned from the network until a network ``core'' is produced.  In the most common case, for some value $k$, nodes whose degree is less than $k$ are pruned (in order of degree) until no more nodes can be removed.  This process was used to model the Internet in \cite{ShaiCarmi07032007} and find key spreaders under the SIR epidemic model in \cite{InfluentialSpreaders_2010}.  More recently, a ``heterogeneous'' version of decomposition was introduced in \cite{baxter11} - in which each node is pruned according to a certain parameter - and the process is studied in that work based on a probability distribution of nodes with certain values for this parameter.

\subsection{Notes on Non-Deterministic Tipping}
We also note that an alternate version of the model where the thresholds are assigned randomly has inspired approximation schemes for the corresponding version of the seed set problem.\cite{kleinberg,leskovec07,chen10}  Work in this area focused on finding a seed set of a certain size that maximizes the expected number of adopters.  The main finding by Kempe et al., the classic work for this model, was to prove that the expected number of adopters was submodular - which allowed for a greedy approximation scheme.  In this algorithm, at each iteration, the node which allows for the greatest increase in the expected number of adopters is selected.  The approximation guarantee obtained (less than $0.63$ of optimal) is contingent upon an approximation guarantee for determining the expected number of adopters - which was later proved to be $\#P$-hard.~\cite{chen10}  Recently, some progress has been made toward finding a guarantee~\cite{Borgs12}.  Further, the simulation operation is often expensive - causing the overall time complexity to be $O(x \cdot n^2)$ where $x$ is the number of runs per simulation and $n$ is the number of nodes (typically, $x>n$).  In order to avoid simulation, various heuristics have been proposed, but these typically rely on the computation of geodesics - an $O(n^3)$ operation - which is also more expensive than our approach.

Additionally, the approximation argument for the non-deterministic case does not directly apply to the original (deterministic) model presented in this paper.  A simple counter-example shows that sub-modularity does not hold here. Sub-modularity (diminishing returns) is the property leveraged by Kempe et al. in their approximation result.

\subsection{Note on an Upper Bound of the Initial Seed Set}

Very recently, we were made aware of research by Daniel Reichman that proves an upper bound on the minimal size of a seed set for the special case of undirected networks with homogeneous threshold values.~\cite{reichman12}  The proof is constructive and yields an algorithm that mirrors our approach (although Reicshman's algorithm applies only to that special case).  We note that our work and the work of Reichman were developed independently.  We also note that Reichman performs no experimental evaluation of the algorithm.

Given undirected network $G$ where each node $v_i$ has degree $d_i$ and the threshold value for all nodes is $k$, Reichman proves that the size of the minimal seed set can be bounded by $\sum_i \min\{1, \frac{k}{d_i+1}\}$.  For our integer tests, we compared our results to Reichman's bound.  Our seed sets were considerably smaller - often by an order of magnitude or more.  See Figure~\ref{fig4a} for details.


